RoboWorM: Evaluating Movement Realism, Consistency and Acceleration Affects in Embodied Video World Models

Video world models (VWMs) are rapidly emerging as scalable neural simulators for robotic manipulation. However, most benchmarks only evaluate them as open-world video generators, using Vision-Language Models (VLMs) that lack strict 3D spatial and kinematic reasoning. To bridge this gap, we introduce RoboWorM, a comprehensive, deployment-aware benchmark that leverages known hardware priors such as robot kinematic trees and fixed camera configurations, to systematically examine structural and spatiotemporal fidelity. RoboWorM curates 1,605 episodes across single-arm, bimanual, and humanoid morphologies, spanning both Markovian and long-horizon non-Markovian tasks under single- and multi-view setups. To explicitly measure physical consistency, we propose two deterministic, VLM-free metrics: KIVA for intra-view kinematic stability, and RIGIS for multi-view geometric consistency. By exploiting intrinsic robotic invariants, KIVA improves hallucination detection alignment with human annotations by 25.8% relative to the strongest frontier VLMs, while RIGIS achieves a 130% higher Spearman correlation with human preferences. Furthermore, since real-world deployment requires low inference latency, we utilize RoboWorM to conduct the first large-scale audit of the quality-efficiency trade-off. Evaluating 9 state-of-the-art acceleration techniques across 3 leading world models (over 29,000 generated rollouts), we demonstrate how these acceleration methods can retain superficial visual quality while silently compromising deployment-critical physical constraints. Using our metrics, we achieve 2.3$\times$ maximum inference speed-up with minimal quality loss.

==> sections/3_method.tex <==

\section{\ours}
\begin{figure}[t]
\centering
\includegraphics[width=0.90\linewidth]{figs/main/dataset_stats.pdf}
\caption{
\textbf{Benchmark Composition and Statistical Breakdown of \ours.} The benchmark aggregates 1,605 episode-camera instances generating 29,343 evaluation rollouts. \textbf{(Top)} Data diversity spans a balanced mix of Markovian (45\%) and non-Markovian (55\%) task dynamics, predominantly multi-view camera setups (79\%), and an even distribution across 5 robot platforms (bimanual, humanoid, and single-arm). \textbf{(Middle)} The acceleration audit covers dense baselines alongside caching (29.6\%), sparse attention (43.2\%), and token reduction (16.4\%) techniques. \textbf{(Bottom)} Representative manipulation primitives encompassing contact-rich actions such as assembly, wiping, and pouring.
\vspace{-0.1in}
}
\label{fig:composition}
\end{figure}


\subsection{Benchmark}
\label{sec:dataset}
\myparagraph{Benchmark Construction.}
\ours{} evaluates the \emph{physical consistency} of generated rollouts under
three sources of variation: embodiment morphology, camera setup, and temporal
dependence. We curate five public teleoperation datasets: DROID~\citep{droid}, RoboChallenge~\citep{robochallenge}, the AIST Bimanual
corpus~\citep{aist2025bimanip}, RoboCOIN~\citep{robocoin}, and NVIDIA GR00T
Teleop GR1~\citep{gao2026dreamdojo}. Together, they yield six
embodiment--camera configurations across five robot platforms and three
morphology classes: single-arm, bimanual, and humanoid, spanning both
single-view and multi-view settings.

Each configuration is further partitioned into \emph{Markovian} and
\emph{non-Markovian} regimes, where the latter requires task history beyond the current observation. In total, the benchmark contains $1{,}608$
episode--camera instances derived from $1{,}308$ distinct trajectories, with
$509$ instructions spanning $14$ manipulation primitives
(\cref{fig:composition}). Dataset-to-configuration mappings, per-cell counts,
regime labeling, and the full curation protocol are provided in
\cref{supp:dataset}.

\myparagraph{World Models under Audit.}
We evaluate three world-model families spanning two diffusion backbone types:
Ctrl-World~\citep{guo2026ctrlworld}, a spatio-temporal U-Net built on Stable
Video Diffusion; DreamGen~\citep{dreamgen}, instantiated with
Cosmos-Predict2 backbones (2B and 14B); and DreamDojo~\citep{gao2026dreamdojo}, an action-conditioned diffusion transformer (2B).

For each supported model configuration pair, we use a checkpoint matched to
the corresponding corpus: nine are fine-tuned by us and three use released
checkpoints. All models are rolled out autoregressively to the ground-truth
episode length at their native training resolution and frame rate, with
identical inputs across generation conditions within each configuration.
Checkpoint details and dense-baseline performance are reported in
\cref{supp:impl_finetuning}.




\subsection{Physics Audit}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/main/metrics.pdf}
    \caption{Caption}
    \label{fig:metrics}
\end{figure}
\subsubsection{KIVA: \underline{K}inematic \underline{I}nvariant \underline{V}iolation \underline{A}ssessment}
% \begin{wrapfigure}{l}{0.45\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{figs/main/kiva2.pdf}
%   \caption{KIVA.}
%   \label{fig:kiva}
% \end{wrapfigure}

\textbf{Diffusion Keypoint Reader.}
A frozen DINOv3 encoder gives patch features $\mathcal F_\tau$ per frame $\tau$.
The reader denoises the coordinates $x_{t,\tau k}$ of keypoint $k$ at noise
level $t$:
\begin{equation}\label{eq:head}
\begin{aligned}
 q_{\tau k}&=\phi(x_{t,\tau k})+\psi(t)+e_k,
 \qquad
 z_{\tau k}=\operatorname{CA}(q_{\tau k},\mathcal F_\tau),\\[2pt]
 \hat x_{0,\tau k}&=x_{t,\tau k}+W_{\mathrm{out}}\operatorname{LN}
 \!\left(z_{\tau k}+\left[\operatorname{TA}(z_{1:T,k}+p_{1:T})\right]_\tau\right),
\end{aligned}
\end{equation}
where $\phi,\psi$ embed coordinate and noise level, $e_k$ is a learned keypoint
identity, $p_{1:T}$ temporal embeddings over the $T$ frames, and
$W_{\mathrm{out}}$ a zero-initialized shared projection. Cross-attention
$\operatorname{CA}$ reads only the tokens of the query's own frame, while
bidirectional temporal attention $\operatorname{TA}$ shares information along a
single keypoint track, letting occluded frames borrow evidence from neighbours.

\textbf{Training and Inference.}
Targets come from the recorded robot state via forward kinematics, normalized to
$[-1,1]^3$, corrupted with Gaussian noise, and recovered under a coordinate-wise
Huber loss $\mathcal L_{\mathrm{kp}}=|\Omega|^{-1}\sum_{i\in\Omega}H_\beta(\hat
x_{0,i}-x_{0,i})$ over all valid coordinates $\Omega$. No bone-length or
smoothness penalty is used, so the properties measured below are never optimized
for. At test time the reader runs ten DDIM updates from Gaussian noise; we
average five samples and invert the normalization to obtain metric positions
$P_{\tau k}$ (Appendix~\ref{supp:kiva}).

\textbf{Kinematic Scores.}
Let $\mathcal B$ hold keypoint pairs whose separation is fixed by the robot
geometry, with nominal length $L_{ab}$, and $\Delta t$ the frame interval:
\begin{equation}\label{eq:detectors}
 r_\tau=10^3\!\!\max_{(a,b)\in\mathcal B}\!
 \left|\,\|P_{\tau a}-P_{\tau b}\|_2-L_{ab}\,\right|,
 \qquad
 j_\tau=\frac{10^3}{\Delta t^{3}}\max_k
 \left\|P_{\tau k}-3P_{\tau-1,k}+3P_{\tau-2,k}-P_{\tau-3,k}\right\|_2 ,
\end{equation}
a link-length error in mm and a third-order jerk in mm/s$^3$. Each 16-frame
segment is summarized by the median $r_\tau$ and the maximum $j_\tau$, then
divided by the $95$th percentile of the same statistic on real videos. The
resulting score is dimensionless: above one means the segment exceeds what real
footage exhibits. Rigidity and jerk are reported separately
(Appendix~\ref{supp:kiva_detectors}).

 
\subsubsection{RIGIS: \underline{R}obotic \underline{I}nter-view \underline{G}eometry \& \underline{I}ntrinsic-extrinsic \underline{S}tability}
\label{sec:rigis}

% \begin{wrapfigure}[22]{l}{0.45\linewidth} 
% \centering 
% \includegraphics[width=\linewidth]{figs/main/rigis.pdf} 
% \caption{\textbf{Overview of RIGIS.} Multi-view inputs are processed via VGGT-$\Omega$ to evaluate geometric consistency $S_{\mathrm{geo}}$ and camera pose stability $S_{\mathrm{pose}}$, yielding the unified metric $S$.}
% \label{fig:rigis} 
% \end{wrapfigure}

Multi-view evaluation faces critical limitations: VLMs struggle with cross-view geometric understanding, while neural 3D estimators, trained on clean data, inadvertently smooth over geometric inconsistencies in generated videos. To bridge this gap, RIGIS establishes an explicit, geometry-grounded evaluation framework. For rigid camera setups, RIGIS evaluates generated multi-view rollouts by ensuring reprojected pixels form a unified 3D scene across views while camera intrinsics and extrinsics remain temporally invariant. At each timestep $i$, the head-modified VGGT-$\Omega$ \citep{} predicts per-view depths and poses, which are scale-aligned, fused, and reprojected into renders $(\bar{X}_i, \bar{D}_i)$ within the visible region.

\textbf{Geometric consistency} measures RGB RMSE $\Delta_X^{(j)}$ and mean absolute depth residual $\Delta_D^{(j)}$ within the visible region, mapped via exponential decay to scores $s_X^{(j)}, s_D^{(j)}$. These are averaged across views and summarized over time as $S_{\mathrm{geo}} = \frac{1}{n}\sum_{i=1}^{n} \prod_{j=1}^{V} \frac{1}{2}(s_X^{(j)}+s_D^{(j)})$.

\textbf{Camera pose stability} computes temporal standard deviations relative to the first frame ($i=0$) for intrinsics ($\sigma_K$) and extrinsic relative pose ($\sigma_R, \sigma_t$). These map to $S_{\mathrm{ext}} = \frac{1}{2}(\mathrm{e}^{-\sigma_R/5}+\mathrm{e}^{-\sigma_t})$ and $S_{\mathrm{int}} = \frac{1}{V}\sum_{j=1}^{V} \mathrm{e}^{-\sigma_K^{(j)}}$, yielding the pose stability score $S_{\mathrm{pose}} = \frac{1}{2}(S_{\mathrm{ext}}+S_{\mathrm{int}})$.

The final RIGIS score $S = \tfrac{1}{2}(S_{\mathrm{geo}} + S_{\mathrm{pose}}) \in [0, 1]$, where a higher score indicates better multi-view consistency. Full details are provided in App.~\ref{supp:metrics_multiview}.

\subsection{Inference Acceleration Methods}






==> sections/tables/speedup.tex <==
% ---------------------------------------------------------------------------
% Speedup table (ICLR 2027, fits the 5.5in text width with \footnotesize).
%
% Preamble requirements:
%   \usepackage{booktabs}
%
% Helper macros (put these in your preamble, or leave them here):
\newcommand{\spx}[1]{#1$\times$}                 % plain speedup
\newcommand{\best}[1]{\textbf{#1$\times$}}        % best per column
\newcommand{\second}[1]{\underline{#1$\times$}}   % second best per column
% ---------------------------------------------------------------------------

\begin{table}[t]
\caption{Inference speedup relative to the dense baseline across three embodiments
(Humanoid, Bimanual, Single-arm) and three world models under multi-view and single-view
settings. \textbf{Best} and \underline{second best} are highlighted. \np{TODO}, \duycomment{Re-structure table as figure with column height for speedup, numbers above for RIGIS/KIVA for multi-view/single-view, the other tables are mean of four metrics. We'll have two figures for one embodiment, one row is about a single view with DreamGen, DreamDoJo, and the bottom row is the multi-view with DreamGen and Ctrl-Word. - Doanh}}
\label{tab:speedup}
\vspace{-0.5em}
\begin{center}
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.1}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}l*{12}{c}@{}}
\toprule
& \multicolumn{4}{c}{\textbf{Humanoid}} & \multicolumn{4}{c}{\textbf{Bimanual}} & \multicolumn{4}{c}{\textbf{Single-arm}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
& \multicolumn{2}{c}{Multi-view} & \multicolumn{2}{c}{Single-view}
& \multicolumn{2}{c}{Multi-view} & \multicolumn{2}{c}{Single-view}
& \multicolumn{2}{c}{Multi-view} & \multicolumn{2}{c}{Single-view} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
\cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
Method & D-Gen & Ctrl-World & D-Gen & D-Dojo & D-Gen & Ctrl-World & D-Gen & D-Dojo & D-Gen & Ctrl-World & D-Gen & D-Dojo \\
\midrule
\textcolor{gray}{Dense}
  & \textcolor{gray}{\spx{1.00}} & \textcolor{gray}{\spx{1.00}} & \textcolor{gray}{\spx{1.00}} & \textcolor{gray}{\spx{1.00}}
  & \textcolor{gray}{\spx{1.00}} & \textcolor{gray}{\spx{1.00}} & \textcolor{gray}{\spx{1.00}} & \textcolor{gray}{\spx{1.00}}
  & \textcolor{gray}{\spx{1.00}} & \textcolor{gray}{\spx{1.00}} & \textcolor{gray}{\spx{1.00}} & \textcolor{gray}{\spx{1.00}} \\
\midrule
SiTo
  & \spx{1.19} & \spx{1.08} & \spx{1.28} & --
  & \spx{1.30} & \spx{1.36} & \spx{1.29} & --
  & \spx{1.17} & \spx{1.01} & \spx{1.29} & -- \\
ITM
  & \spx{1.16} & \spx{1.05} & \spx{1.15} & --
  & \spx{1.06} & \spx{1.32} & \spx{1.15} & --
  & \spx{1.16} & \spx{1.07} & \spx{1.18} & -- \\
\midrule  % optional group separator (token pruning / caching / sparse attention)
WorldCache
  & \best{2.28} & \best{1.94} & \best{1.95} & \best{1.82}
  & \best{1.76} & \best{2.24} & \best{1.35} & \second{1.65}
  & \best{2.28} & \best{1.81} & \best{1.58} & \best{1.73} \\
DiCache
  & \second{2.08} & \second{1.84} & \second{1.89} & \second{1.72}
  & \second{1.66} & \second{2.04} & \second{1.32} & \best{1.67}
  & \second{2.08} & \second{1.74} & \second{1.53} & \second{1.65} \\
FasterCache
  & \spx{1.46} & -- & \spx{1.45} & \spx{1.32}
  & \spx{1.29} & -- & \spx{1.27} & \spx{1.22}
  & \spx{1.46} & -- & \spx{1.21} & \spx{1.32} \\
\midrule  % optional group separator
PISA
  & \spx{1.44} & \spx{1.34} & \spx{1.45} & \spx{1.06}
  & \spx{1.46} & \spx{1.22} & \spx{1.14} & \spx{1.03}
  & \spx{1.32} & \spx{1.32} & \spx{1.37} & \spx{1.05} \\
Radial
  & \spx{1.36} & \spx{1.32} & \spx{1.36} & \spx{1.07}
  & \spx{1.41} & \spx{1.16} & \spx{1.10} & \spx{1.02}
  & \spx{1.29} & \spx{1.28} & \spx{1.34} & \spx{1.07} \\
Single-viewG1
  & \spx{1.29} & \spx{1.19} & \spx{1.28} & \spx{1.11}
  & \spx{1.45} & \spx{1.08} & \spx{1.15} & \spx{1.15}
  & \spx{1.22} & \spx{1.15} & \spx{1.39} & \spx{1.14} \\
Single-viewG2
  & \spx{1.19} & \spx{1.17} & \spx{1.15} & \spx{1.07}
  & \spx{1.40} & \spx{1.15} & \spx{1.12} & \spx{1.15}
  & \spx{1.16} & \spx{1.13} & \spx{1.26} & \spx{1.24} \\
\bottomrule
\end{tabular}}
\end{center}
\end{table}
